Optimal Static Dictionary with Worst-Case Constant Query Time

In this paper, we design a new succinct static dictionary with worst-case constant query time. A dictionary data structure stores a set of key-value pairs with distinct keys in $[U]$ and values in $[\sigma]$, such that given a query $x\in [U]$, it quickly returns if $x$ is one of the input keys, and if so, also returns its associated value. The textbook solution to dictionaries is hash tables. On the other hand, the (information-theoretical) optimal space to encode such a set of key-value pairs is only $\text{OPT} := \log\binom{U}{n}+n\log \sigma$. We construct a dictionary that uses $\text{OPT} + n^{\epsilon}$ bits of space, and answers queries in constant time in worst case. Previously, constant-time dictionaries are only known with $\text{OPT} + n/\text{poly}\log n$ space [P\v{a}tra\c{s}cu 2008], or with $\text{OPT}+n^{\epsilon}$ space but expected constant query time [Yu 2020]. We emphasize that most of the extra $n^{\epsilon}$ bits are used to store a lookup table that does not depend on the input, and random bits for hash functions. The "main" data structure only occupies $\text{OPT}+\text{poly}\log n$ bits.

==> concat1.tex <==
\subsubsection{Storing variable-length parts}
\label{subsubsection:storing_varlength}

We formulate the problem of storing the variable-length parts as a retrieval problem. A key in this retrieval problem can be described as a tuple $(i,j)\in [L]\times [M_{\max}-M_{\min}]$. The key $(i,j)$ is present in the problem if the variable-length part of $M_i$ has length at least $j$, and the value in this case would be the content of $j$-th word in the variable-length part of $M_i$. When the algorithm needs to access some word in the variable-length part (after knowing the corresponding $s_i$ and therefore $M_i$), it just asks the retrieval data structure with the corresponding key.

We will use \cref{thm:augmented_retrieval} to solve this problem. The algorithm uses part of $m_{\text{fixed}}$ as the augmented array. In particular, the algorithm will take the first
$$
3L(M_{\max}-M_{\min})\log\bk*{L(M_{\max}-M_{\min})}
$$
words of $m_{\text{fixed}}$, and combine them with the queries from $[L]\times [M_{\max}-M_{\min}]$ to form an augmented retrieval problem. 

Under the cell-probe model, the algorithm applies \cref{thm:augmented_retrieval} to solve this retrieval problem over the field $GF(2^w)$. The operations on $GF(2^w)$ can be performed in constant time with a lookup table, which does not count as spaces in the cell-probe model.\zjkcomment{In cell-probe, field operation only has O1 cost ...} Later when handling the RAM model, the algorithm will use the technique in \cref{subsubsection:storing_spills} to round up the field size to the closest prime and use the solution there for this part.\sidenote{If we want to focus on cell-probe here, then even don't mention ``constant time'' or ``lookup tables''.}

For answering the queries, if the algorithm needs to access the variable-length part, or part of $m_{\text{fixed}}$ used as the augmented array here, it will query the augmented retrieval data structure and get the result in constant time. The memory overhead produced in this part is $O(1)$ words caused by the augmented retrieval problem.\sidenote{The augmented retrieval does not claim to waste any bit, and it succeeds with a constant probability. Something is missing in between.}


==> concat2.tex <==
\subsubsection{Storing spills}
\label{subsubsection:storing_spills}
\note{Either change the two subsubsections to paragraphs, or make sure the last subsubsection is ended properly with another (sub)subsection.}

The last step is to store the spills $k_i$ produced by each bucket. If all $k_i$ belong to the same universe $\Sigma$, then we can solve this problem using techniques from \cite{dodis2010changing}:

\begin{theorem}[{\cite[Theorem 1]{dodis2010changing}}]\label{thm:changing_base}
On a Word RAM, one can represent a vector $A[1 . . n]$ of elements from a finite alphabet $\Sigma$ using $\lceil n \log_2 \Sigma\rceil$ bits, such that any element of the vector can be read or written in constant time. The data structure requires
$O(\log n)$ precomputed word constants.
\end{theorem}

However, in our setting, different buckets could have different universe sizes $K_i$, so we cannot apply the theorem above directly.

Our solution is as follows. Since the number of different $s_i$'s is small, we group buckets by their sizes $s_i$ and store each group separately. Similar to \cref{subsubsection:storing_varlength}, the problem of storing spills in each group $s$ can be viewed as a retrieval problem: The keys are indices $i$ in this group, the associated value for key $i$ is $k_i$, and the universe of values is $[K^{(s)}]$. We use \cref{thm:augmented_retrieval} to solve this problem in some field $\F$, then use \cref{thm:changing_base} to store the cell content of the augmented retrieval data structure.\sidenote{This seems under-detailed. Maybe use more words to explain about \cref{thm:changing_base}.}

There are still a few problems left over. First, the augmented retrieval problem needs a field $\F$ that can hold $[K^{(s)}]$, but a finite field of size $K^{(s)}$ may not exist unless $K^{(s)}$ is a prime power. To deal with this issue, we need choose the smallest prime $P^{(s)}$ larger than $K^{(s)}$, and use $\F_{P^{(s)}}$ as our field, but this step leads to extra redundancy. Fortunately, the following lemma bounds the gap from $K^{(s)}$ to the next prime $P^{(s)}$ and the redundancy.

\begin{lemma}[\cite{NextPrime}]\label{lem:nextprime}
    For sufficiently large $n$, there exists a prime in $[n, \, n+n^{7/11}]$.
\end{lemma}

The next problem is that, the augmented retrieval data structure under $\F_{P_i}$ needs an augmented array in field $\F_{P^{(s)}}$. However, $m_{\text{fix}}$ are stored in words with base $2^w$, and we must convert from base $2^w$ to base $P^{(s)}$. \cref{thm:changing_base} only supports converting from arbitrary bases to base $2^w$, but a closer look into their proof\zjkcomment{Is this right?} shows that their method also works for changing to other large-enough bases.

\begin{corollary}\label{changing_base_2}
For any two bases $p,q\in poly(n)$ and $q\geq n^2$, we can storing a sequence $A[1\cdots n]$ of base $p$ by a sequence $B$ that can holds elements in $
\F_q$, such that
\begin{itemize}
    \item The redundancy is $O(1)$ words and a look-up table of $O(\log n)$ words.
    \item Each element in $A$ can be restored by accessing constant number of elements in $B$ and using constant time.
\end{itemize}
\end{corollary}
\note{Renfei: I think this should be combined with the original theorem, i.e., when stating the original theorem, directly state this generalized version. Maybe add a footnote to explain what was generalized.}

\note{General comment: Watch the wording -- do not ``build a problem''.}

By this result, we could solve the retrieval for each kind of $[P^{(s)}]$ as follows: First convert part of $m_{\text{fix}}$ into elements in $[P^{(s)}]$, use them to build the augmented retrieval under $\F_{P^{(s)}}$, and finally convert the retrieval data structure back to word representation. In particular, our algorithm will do the following steps for each $s\in[B_{\min}, B_{\max}]$.

\begin{itemize}
    \item Take the next $60L \log L$ words in $m_{\text{fix}}$ that are not used in the previous steps of the construction, and convert this sequence to base $P^{(s)}$ using \cref{changing_base_2}. Let the resulting sequence be $m_{\text{conv}}^{(s)}$. Since $P^{(s)}$ is bounded by $2M^{(s)}$ using \cref{lem:nextprime}, the length of $m_{\text{conv}}^{(s)}$ is at least $3L\log L$.\sidenote{This reasoning is not clear. Why the output length is at least $3L \log L$?}
    \item Construct an augmented retrieval data structure in $\F_{P^{(s)}}$ using $(i,k_i)$ for indices in this group\sidenote{What are ``indices in this group''? Is this term defined?} as keys and values, with $m_{\text{conv}}^{(s)}$ as the augmented array. The requirement in \cref{thm:augmented_retrieval} is satisfied since the number of possible queries is $L$.\sidenote{What requirement?} The augmented retrieval data structure built can be represented as a sequence of elements in $\F_{P^{(s)}}$. Let this sequence be $m_{\text{retr}}^{(s)}$.
    \item Convert $m_{\text{retr}}^{(s)}$ back to words using \cref{changing_base_2} again, then store these words sequentially.
\end{itemize}

\note{Adding a picture may help illustrate the process.}

Next, we consider handling the queries.\sidenote{Not enough set-up for queries. What queries are we talking about?} If the algorithm needs to access part of $m_{\text{fix}}$ used in the above construction, it first goes through the algorithm of converting from $m_{\text{fix}}$ from $m_{\text{conv}}^{(s)}$\sidenote{Typo here, can't understand}, and \cref {changing_base_2} shows that each element in $m_{\text{fix}}$ can be restored by accessing constant number of elements in $m_{\text{conv}}^{(s)}$. Each access is a query of the augmented array in the augmented retrieval data structure, and the algorithm needs to access constant number of elements in $m_{\text{retr}}^{(s)}$ in each query. Each access of $m_{\text{retr}}^{(s)}$ can be performed in constant time by again following the base-conversion process from $m_{\text{retr}}^{(s)}$ to words. The overall process takes constant time, so each query to the fixed-length part only needs constant time.\sidenote{This paragraph will be more clear if there is a figure.}

If the algorithm needs to access some spill $k_i$, it first tries to find the bucket size $s_i$ by query the bucket. The construction in \cref{lem:bucket_rep} shows that this can be performed by querying the first word of $m_i$. The algorithm then uses $s_i$ to find the corresponding augmented retrieval data structure and queries the data structure. Similar to the analysis above, a query is performed by accessing $m_{\text{retr}}^{(s)}$ for constant times, where each access can be performed in constant time.

By combining this construction with \cref{subsubsection:storing_varlength}, we store all $(m_i,k_i)$ in words, supporting constant-time querys on them. We now prove the complete correctness of this algorithm.


==> prelim.tex <==
bla bla, spill-over representation, length of $(M,K)$ is defined as $M+\log K$. Without further specification, $K$ is always $\poly n$.

Matrix notations: $M_{S,T}$ is the submatrix of $M$ with rows $S$ and columns $T$, $M_{S,*}$ is the submatrix of $M$ with rows $S$ and all the columns.


